Large Language Models at Work in China's Labor Market

This paper explores the potential impacts of large language models (LLMs) on the Chinese labor market. We analyze occupational exposure to LLM capabilities by incorporating human expertise and LLM classifications, following the methodology of Eloundou et al. (2023). The results indicate a positive correlation between occupational exposure and both wage levels and experience premiums at the occupation level. This suggests that higher-paying and experience-intensive jobs may face greater exposure risks from LLM-powered software. We then aggregate occupational exposure at the industry level to obtain industrial exposure scores. Both occupational and industrial exposure scores align with expert assessments. Our empirical analysis also demonstrates a distinct impact of LLMs, which deviates from the routinization hypothesis. We present a stylized theoretical framework to better understand this deviation from previous digital technologies. By incorporating entropy-based information theory into the task-based framework, we propose an AI learning theory that reveals a different pattern of LLM impacts compared to the routinization hypothesis.

==> img_exposure_tex/ai_exposure_expert.tex <==
\begin{figure}[htb]
\begin{centering}
\includegraphics[width=0.95\linewidth]{./img_exposure/fig_ai_exposure_expert.png}
\par\end{centering}
\caption{AI Occupation Exposure: Expert.}
\label{fig:ai_exposure_expert}
\end{figure}


==> img_exposure_tex/change_share_vancancy.tex <==
\begin{figure}[htb]
\begin{centering}
\includegraphics[width=0.95\linewidth]{./img_exposure/fig_change_share_vancancy.png}
\par\end{centering}
\caption{Percentage Change of Share of Vacancy of Large-category Occupations.}
\label{fig: percentage change of share vacancy}
\end{figure}

==> img_exposure_tex/econ_growth.tex <==
\begin{figure*}[htb]
\begin{centering}
\includegraphics[width=0.65\linewidth]{./img_exposure/fig_econ_growth}
\par\end{centering}
\caption{Contour curve of economic growth with respect to sector technology adoption ratio and damage ratio (where $\rho=1$). The sectors are sorted in decreasing order of AI industry exposure $r_i$.}
\label{fig:contour_plots_econ_growth}
\vspace{-1.2em}
\end{figure*}


==> img_exposure_tex/large_score_GLM2+Internlm.tex <==
\begin{figure}[htb]
\begin{centering}
\includegraphics[width=0.95\linewidth]{./img_exposure/fig_large_score_GLM2+Internlm.png}
\par\end{centering}
\caption{AI Large-category Occupation Exposure: GLM2+InternLM.}
\label{fig:large_score_GLM2+Internlm}
\end{figure}

==> img_exposure_tex/large_score_GPT.tex <==
\begin{figure}[htb]
\begin{centering}
\includegraphics[width=0.95\linewidth]{./img_exposure/fig_large_score_GPT.png}
\par\end{centering}
\caption{AI Large-category Occupation Exposure: GPT.}
\label{fig:large_score_GPT}
\end{figure}

==> img_exposure_tex/medium_GLM2+Internlm.tex <==
\begin{figure}[htb]
\begin{centering}
\includegraphics[width=0.95\linewidth]{./img_exposure/fig_medium_GLM2+Internlm.png}
\par\end{centering}
\caption{AI Medium-category Occupation Exposure: GLM2+InternLM.}
\label{fig:medium_score_GLM2+Internlm}
\end{figure}

==> img_exposure_tex/medium_GPT.tex <==
\begin{figure}[htb]
\begin{centering}
\includegraphics[width=0.95\linewidth]{./img_exposure/fig_medium_GPT.png}
\par\end{centering}
\caption{AI Medium-category Occupation Exposure: GPT.}
\label{fig: medium_score_GPT}
\end{figure}

==> img_exposure_tex/share_vacancy.tex <==
\begin{figure}[htb]
\begin{centering}
\includegraphics[width=0.95\linewidth]{./img_exposure/fig_share_vacancy.png}
\par\end{centering}
\caption{Share of Vacancy of Large-category Occupations: 2017-2022.}
\label{fig: share vacancy}
\end{figure}

==> img_exposure_tex/vacancy_score.tex <==
\begin{figure}[htb]
\begin{centering}
\includegraphics[width=0.95\linewidth]{./img_exposure/fig_vacancy_score.png}
\par\end{centering}
\caption{AI Exposure on Vacancy Structure.}
\label{fig: ai exposure on vacancy}
\end{figure}
